On Optimizing the Trade-off between Privacy and Utility in Data Provenance

Organizations that collect and analyze data may wish or be mandated by regulation to justify and explain their analysis results. At the same time, the logic that they have followed to analyze the data, i.e., their queries, may be proprietary and confidential. Data provenance, a record of the transformations that data underwent, was extensively studied as means of explanations. In contrast, only a few works have studied the tension between disclosing provenance and hiding the underlying query. This tension is the focus of the present paper, where we formalize and explore for the first time the tradeoff between the utility of presenting provenance information and the breach of privacy it poses with respect to the underlying query. Intuitively, our formalization is based on the notion of provenance abstraction, where the representation of some tuples in the provenance expressions is abstracted in a way that makes multiple tuples indistinguishable. The privacy of a chosen abstraction is then measured based on how many queries match the obfuscated provenance, in the same vein as k-anonymity. The utility is measured based on the entropy of the abstraction, intuitively how much information is lost with respect to the actual tuples participating in the provenance. Our formalization yields a novel optimization problem of choosing the best abstraction in terms of this tradeoff. We show that the problem is intractable in general, but design greedy heuristics that exploit the provenance structure towards a practically efficient exploration of the search space. We experimentally prove the effectiveness of our solution using the TPC-H benchmark and the IMDB dataset.

==> np_hardness.tex <==
\begin{figure}[h]
    \centering \footnotesize
    \begin{tabular}{| c | c |} 
        \hline Output & Provenance \\ [0.5ex]
        \hline $e_1, \ldots, e_m$ & $VC_1 \cdots VC_{N}$\\ 
        \hline $1, \ldots, 1$ & $yes^k \cdot no^{N-k}$\\ 
        \hline
    \end{tabular}
\caption{\ex\ for NP-hardness proof} \label{fig:hardness_example}
\end{figure}

We define the decision problem version of the optimal abstraction such that, given an abstraction tree compatible with a \ex\ and integers $k, l$, the solution is an abstraction function that gives a privacy of at least $k$ with at most $l$ loss of information. 

\begin{proposition}\label{prop:hardness}
The decision problem version of the optimal abstraction is NP-hard. 
\end{proposition}

\begin{proof}
We show that the problem is NP-hard by reduction from the decision problem version of Vertex Cover. The input to Vertex Cover is a graph $G = (V,E)$, where $|V| = n, |E| = m$ and an integer $k \in \mathbb{N}$, and the solution is a set of vertices $C \subseteq V$ such that $\forall e \in E.~ C\cap e \neq \emptyset$. 

Given such an input, we define the relation $VC(V,E,N)$ where $(v_i, e_j, 2) \in VC$ iff $v_i \in e_j$ (these tuples are denoted by $VC_1, \ldots, VC_N$). 
$VC$ also contains the additional two tuples $(0,1,3), (0,0,3)$, denoted by $yes, no$ respectively. 
Denote by $N+2$ the number of tuples in $VC$.
We then define a \ex\ $Ex$ with two rows as seen in Figure \ref{fig:hardness_example}. The constant $2$ and $3$ are there to make sure we generate connected queries as part of the reduction.
We also define the abstraction tree to be $T$ where $L(T) = VC_1, \ldots, VC_N$ and each $VC_i$ is connected to a node $VC(\widetilde{v},\widetilde{e}, 2)$, where the weight of each edge is $1$ \amir{or something with entropy}. 

Now, we claim that $G$ has a cover of size at most $k$ iff there is an  abstraction function that gives privacy at least $k$ with at most $N-m$ loss of information. 

($\Leftarrow$) Suppose we have an abstraction function $A_T$ that gives privacy at least $k$ with at most $N-m$ loss of information. Let $Q$ be a CIM query w.r.t. $A_T(Ex)$. In particular, $Q$ is consistent w.r.t. a certain concretization of $A_T(Ex)$ (Definition \ref{def:consistent}). Assume that the monomial in the first row of this concretization is $VC_1'\cdots VC_N'$. Given this concretization, $Q$ should generate $e_1,\ldots, e_m$ from this monomial and $1, \ldots, 1$ from the second monomial. Therefore, $Q$ has to map the same $k$ projected atoms to the tuples $yes^k$ and to some $k$ tuples $VC_{i_1}'\cdots VC_{i_k}'$. We choose the vertices represented by $VC_{i_1}'\cdots VC_{i_k}'$ as the vertex cover for the graph $G$. Since every edge is covered (as the output of $Q$ is the tuple $(e_1, \ldots, e_m)$), this is indeed a cover of size $k$. 

($\Rightarrow$) Suppose we have a cover of size $\leq k$, $\{v_1, \ldots, v_k\}$. 
We show how to generate an abstraction function from this cover. 
For every $v_i \in \{v_1, \ldots, v_k\}$, and the edge covered by it $e_j$ we {\em do not} abstract $VC(v_i, e_j, 2)$ (there are a total of $m$ such tuples, one for each edge).
For every other tuple tuple $VC(v_i', e_j', 2)$, replace it with its abstraction $VC(\widetilde{v},\widetilde{e}, 2)$. We get $\absEx{Ex}$ where $N-m$ tuples are abstracted to the same tuple $VC(\widetilde{v},\widetilde{e}, 2)$. 
Note that for each $v_i \in \{v_1, \ldots, v_k\}$ covering $e_j$, we have a concretization of $\absEx{Ex}$ such that:
\begin{center}
\begin{footnotesize}
\begin{tabular}{| c | c |} 
        \hline Output & Provenance \\ [0.5ex]
        \hline $e_1, \ldots, e_m$ & $VC_1\cdots VC_m\cdot VC_i^{N-m}$\\ 
        \hline $1, \ldots, 1$ & $yes^m \cdot no^{N-m}$\\ 
        \hline
\end{tabular}
\end{footnotesize}
\end{center}

From this concretization we can generate the CIM query 
$$Q(x_1, \ldots, x_m) :- VC(y_1, x_1, z), \ldots, VC(y_k, x_m, z), VC^{N-m}(y_i, w, z)$$ 
i.e., a query that maps the first $k$ atoms to the tuples that cover show which vertex covers which edge and another atom that can be mapped to the rest of the $N-k$ tuples. We have $k$ such different concretizations such that each produces a distinct query with this structure. Since each such concretization results in a different CIM query, we have privacy of $\geq k$. Additionally, we have abstracted $N-m$ tuples, so out loss of information is $N-m$ as per the number of edges we have used. 
\end{proof}
